An Exploratory Analysis on Users' Contributions in Federated Learning

Federated Learning is an emerging distributed collaborative learning paradigm adopted by many of today's applications, e.g., keyboard prediction and object recognition. Its core principle is to learn from large amount of users data while preserving data privacy by design as collaborative users only need to share the machine learning models and keep data locally. The main challenge for such systems is to provide incentives to users to contribute high-quality models trained from their local data. In this paper, we aim to answer how well incentives recognize (in)accurate local models from honest and malicious users, and perceive their impacts on the model accuracy of federated learning systems. We first present a thorough survey on two contrasting perspectives: incentive mechanisms to measure the contribution of local models by honest users, and malicious users to deliberately degrade the overall model. We conduct simulation experiments to empirically demonstrate if existing contribution measurement schemes can disclose low-quality models from malicious users. Our results show there exists a clear tradeoff among measurement schemes in terms of the computational efficiency and effectiveness to distill the impact of malicious participants. We conclude this paper by discussing the research directions to design resilient contribution incentives.

==> Sections/Introduction_.tex <==

%-------------------------------------------------------------------------------%
%-------------------------------------------------------------------------------%
\section{Introduction}
\label{sec:Introduction}
%-------------------------------------------------------------------------------%
%-------------------------------------------------------------------------------%
\gill {intro on FL}

Recent progresses in deep learning have forwarded breakthroughs in both academic research and practical applications \cite{yao2019revisiting}. Generally, deep learning models require a large number of centralized authentic data to train neural network models of high performance. However, due to the privacy rules by the European Union’s General Data Protection Regulation (GDPR), security and privacy demands poses restrictions on benefits of related AI technologies. While collecting sensitive information such as personal photos and sounds, especially financial and health data, raises legislative challenges. With the significant improvement of data scale and computing power, Federated learning (FL) has become an attractive solution \cite {yang2019federated} for privacy preserving distributed deep learning framework with abundant achievements academically \cite{wang2019edge}\cite{wei2019multi} and systematically\footnote{https://github.com/FederatedAI/FATE}.
% enabling multiple participants to collaboratively learn a centralized global model 
 Federated Learning enables multiple participants to collaboratively learn a centralized global model from distributed training data according to their own input without sharing private data (as shown in Figure \ref{fl}). The typical difference between federated learning and distributed learning lies in the assumptions made on the properties of the local datasets,\cite{Konecny:2015:corr:optimization} as distributed learning originally aims at parallelizing computing power 
while federated learning for training on heterogeneous datasets.

 
\begin{figure}
\setlength{\abovecaptionskip}{-0cm}   %调整图片标题与centering
\includegraphics[height=7.0cm]{./Figures/fl.png}
\caption{Introduction of Federated Learning}
\label{fl}
\end{figure}

\textbf{Definition:} Federated learning is a machine learning setting where multiple entities (clients) collaborate in solving a machine learning problem, under the coordination of a central server or service provider. Each client’s raw data is stored locally and not exchanged or transferred; instead, focused updates intended for immediate aggregation are used to achieve the learning objective \cite{Kairouz:2019:corr:advance}. 



 From Figure \ref{fl_pro} we can explain classical FL system in detail, this iterated procedure can be summarized as four steps: 
\textbf{Initialization:} The server defines a specific machine learning task and initialize network parameters ready as basic model. \textbf{Client Selection:} In order to perform superiority of data diversity, FL server tends to choose clients with good network connection randomly to train their local model. \textbf{Local Training:} Selected clients receive basic model from server and train local model using their own data. \textbf{Secure Aggregation:} The server averages neural network parameter updates uploaded from clients without access to their local data. All steps but Initialization are iterated until the global model achieves a desired performance.
 
  
\begin{figure}
\setlength{\abovecaptionskip}{-0cm}   %调整图片标题与centering
\includegraphics[height=9.0cm]{./Figures/fl_protocal.png}
\caption{Protocol of Federated Learning}
\label{fl_pro}
\end{figure}
 
 
%  The typical difference between federated learning and distributed learning lies in the assumptions made on the properties of the local datasets,\cite{Konecny:2015:corr:optimization} as distributed learning originally aims at parallelizing computing power where federated learning originally aims at training on heterogeneous datasets. While distributed learning also aims at training a single model on multiple servers, a common underlying assumption is that the local datasets are identically distributed (i.i.d.) and roughly have the same size. None of these hypotheses are made for federated learning; instead, the datasets are typically heterogeneous and their sizes may span several orders of magnitude. Moreover, the clients involved in federated learning may be unreliable as they are subject to more failures or drop out since they commonly rely on less powerful communication media (i.e. Wi-fi) and battery-powered systems (i.e. smartphones and IoT devices) compared to distributed learning where nodes are typically datacenters that have powerful computational capabilities and are connected one another with fast networks \cite{Kairouz:2019:corr:advance}.

However, due to the self-interest clients in crowdsourcing scenarios, FL systems are supposed to involve incentive mechanism to attract clients of high quality and build ecosystems. On the other hand, since there are incentives as monetary rewards, selfish and malicious clients would absolutely misbehave to gain more profits or even damage the whole system. Thus, this paper is focusing on a contrasting view on attacks and incentives of federated learning. The contribution of this paper could be summarized as follows:
 \begin{itemize}
     \item We provide a comprehensive survey summarizing the SOTA attacks and incentives of federated learning, and propose a formal definition of FL incentive mechanism.
     \item We implement some typical contribution evaluation metrics of incentive mechanism to demonstrate how it will recognize malicious participants. 
     \item Visions on possible attacks for the weaknesses of existing incentive mechanisms to cheat for higher rewards have been proposed, as well as the future research directions of incentives.
 \end{itemize}



==> Sections/ResearchDirections_.tex <==
%-------------------------------------------------------------------------------%
%-------------------------------------------------------------------------------%
\section{Discussion and Research Directions}
\label{sec:ResearchDirections}
%-------------------------------------------------------------------------------%
%--

\rania{This is temporary content until better ideas come up}
\subsection{Possible Attacks for Contribution Evaluation Strategies}
%do we need to combine this subsetion with Contribution Evaluation Taxonomy?
\begin{itemize}
    \item \textbf{Attacks Against Marginal-Loss Based Contribution Evaluation :} A possible attack against marginal-loss-based contribution evaluation mechanisms would be a causative training-time attack where a free-rider aims at having high participation rewards without holding good quality data of its own. The latter has white-box access to the model along with a background testing dataset. We also assume that this attacker can intercept certain local model updates sent to the federator by eavesdropping the network. To carry out his attack during federated learning round, a free-rider would first generate class-representatives out of the current version of the model via a GAN-based approach. After that, as soon as the new round starts, he eavesdrops parts of the network during a small time period and intercepts a small subset of local updates sent by some of the clients selected by the federator. The latter uses these intercepted updates to have an estimate of the influence value attributed to him by the federator. To do that, he keeps updating the class representatives he previously generated with randomly added noise while maximizing the estimated influence. This process is repeated for a reasonable number of iterations. Finally, the attacker reports the optimal update to the federator before the reporting-time threshold exceeds.
    \item \textbf{Attacks Against Similarity-Based Contribution Evaluation : }
    Similarity-based contribution evaluation mechanisms can be attacked by a free-rider by generating class-representatives based on past-observations of the model since this knowledge is for sure captured by the local-models of the versifiers, this would help the attacker to get high similarity rate between his generated labels and the once obtained by verifiers via classification.
\end{itemize}
\gill {Research Direction of incentive}


\subsection{Possible Research Directions for incentive design}
\subsubsection{\textbf{Fairness in Federated Learning}}
Federated learning ecosystem requires well-built fairness such as Collaborative fairness\cite{Lyu:2019:iacr:Towards} for reward distribution, Waiting regret fairness\cite{yu:2020:AIES:fair} for settlement delay. Different fairness organization in federated learning systems hold disparate impact on the system characteristics, so as to distinctive participants. Future research on incentive mechanism could focus on the definition of fairness under various of application scenarios of federated learning.
\subsubsection{\textbf{Leverage IID and Diversity}}
The basic idea of Federated Learning is to surmount the difficulty of data isolation. Multiple participants contribute their data to collaboratively train a global model. The diversity of data among clients are in need to train a model without bias. However, owing to the fact that global learning model collect data across the FL network in a Non-IID (Non-Independent and Identically Distributed) manner via numerous, or even anonymous clients, the global model may suffer from convergence difficulty. Therefore, further study on leveraging IID and Diversity of FL clients would see the significant nature behind it.
\subsubsection{\textbf{Make Incentive Schemes Efficient}}
Researches on incentive mechanism design of federated learning is still at the early stage, and most fascinating outcomes have involve heavy computation overhead or massive parameter transmission. For instance, similarity-based contribution measurements \cite{Kang:2019:IEEEIoT:contract} include broadcasting among clients with different submission time, while introducing blockchain as reliable reputation records to enhance fairness. Prospective studies on incentive may not ignore this challenge: make the incentive design both effective and efficient.
